Average site perimeter of directed animals on the two-dimensional lattices

We introduce new combinatorial (bijective) methods that enable us to compute the average value of three parameters of directed animals of a given area, including the site perimeter. Our results cover directed animals of any one-line source on the square lattice and its bounded variants, and we give counterparts for most of them in the triangular lattices. We thus prove conjectures by Conway and Le Borgne. The techniques used are based on Viennot's correspondence between directed animals and heaps of pieces (or elements of a partially commutative monoid).

==> applications.tex <==
\section{Applications}\label{section:applications}

\subsection{Asymptotic results}

\begin{lemma}
For all $m\geq0$, the polynomials $F_m(t)$ and $\widehat F_m(t)$ have only
real, simple roots. Their respective smallest root are given by:
\begin{align*}
\frac1{\rho_m}&=4\cos^2\frac\pi{m+2}\text;\\
\frac1{\sigma_m}&=4\cos^2\frac\pi{2m}\text.
\end{align*}
\end{lemma}


\begin{proof}
We check by induction on $m$ that the degrees of $F_m(t)$ and $\widehat
F_m(t)$ are \smash{$\bigl\lceil\frac m2\bigr\rceil$} and
\smash{$\bigl\lfloor\frac m2\bigr\rfloor$}, respectively. We also check by
induction the following identities:
\begin{align*}
F_m\biggl(\frac1{4\cos^2\theta}\biggr)&=
\frac{\sin[(m+2)\theta]}{(2\cos\theta)^{m+1}\sin\theta}\text;\\
\widehat F_m\biggl(\frac1{4\cos^2\theta}\biggr)&=
\frac{2\cos(m\theta)}{(2\cos\theta)^{m}}\text.
\end{align*}
By choosing appropriate values of $\theta$ in the interval $[0,\pi/2)$, these
identities account for all the roots of the polynomials. Thus, we prove that
the roots are real and simple, and we derive the value of the smallest root.
\end{proof}

Let now $\Gamma$ be a square lattice and $\Delta$ its associated triangular
lattice, and let $S$ be a one-line source. We denote by $a(n)$ and $\bar a(n)$
the number of animals of source $S$ with area $n$ on $\Gamma$ and $\Delta$,
respectively.

Using singularity analysis \cite{flajolet} on the results of
Section~\ref{section:dominoes}, we find estimates for these numbers as $n$
tends to infinity:
\begin{align*}
a(n)&\sim\lambda\mu^nn^\gamma\text;&
\bar a(n)&\sim\bar\lambda\bar\mu^nn^\gamma\text.
\end{align*}
In the triangular lattices, the growth constant $\bar\mu$ is 4 on the
unbounded lattices, $\frac1{\rho_m}$ on the rectangular lattice of width~$m$,
and $\frac1{\sigma_m}$ on the cylindrical lattice of width~$m$; on the square
lattices, the growth constant $\mu$ is equal to $\bar\mu-1$. The constant
$\gamma$ is $-1/2$ on the full lattice, $-3/2$ on the half lattice, and $1$ on
the bounded lattices. Finally, the factors $\bar\lambda$ and $\lambda$ depend
on the source $S$.


\begin{corollary}
Assume that $\Gamma$ is either the full lattice, the half lattice, or a
cylindrical bounded lattice. As $n$ tends to infinity, we have the following
estimates:
\begin{align*}
j(n)&\sim\frac n{\mu+1};&\bar\jmath(n)&\sim\frac n{\bar\mu+1}\text;\\
\ell(n)&\sim\frac n{\mu^2};&\bar\ell(n)&\sim\frac n{\bar\mu(\bar\mu+1)}\text;\\
p_i(n)&\sim p_e(n)\sim\frac\mu{\mu+1}n\text.
\end{align*}
\end{corollary}

In the unbounded lattices, the growth constants are $\mu=3$ and $\bar\mu=4$.
Thus, these estimates become:
\begin{align*}
j(n)&\sim\frac n4;&\ell(n)&\sim\frac n9;&p(n)&\sim\frac{3n}4;&
\bar\jmath(n)&\sim\frac n5;&\bar\ell(n)&\sim\frac n{20}.
\end{align*}

\begin{proof}
In the full, half, and cylindrical models, the position $q+2$ is always in
$Q$ as soon as $q$ is. This means that in these models, the generating
function $M_{[S]}(t)$ (see Definition~\ref{definition:square2}) simply counts
animals marked with any site. Its $n$th coefficient is $na(n)$.
\end{proof}

\subsection{Examples}

\[P^e(t)=D_m(t)+\frac{t}{1+t}D_m'(t)+\frac1{1+t}D_m(t)^2.\]




